Convergence and Stability of Graph Convolutional Networks on Large Random Graphs

We study properties of Graph Convolutional Networks (GCNs) by analyzing their behavior on standard models of random graphs, where nodes are represented by random latent variables and edges are drawn according to a similarity kernel. This allows us to overcome the difficulties of dealing with discrete notions such as isomorphisms on very large graphs, by considering instead more natural geometric aspects. We first study the convergence of GCNs to their continuous counterpart as the number of nodes grows. Our results are fully non-asymptotic and are valid for relatively sparse graphs with an average degree that grows logarithmically with the number of nodes. We then analyze the stability of GCNs to small deformations of the random graph model. In contrast to previous studies of stability in discrete settings, our continuous setup allows us to provide more intuitive deformation-based metrics for understanding stability, which have proven useful for explaining the success of convolutional representations on Euclidean domains.

==> future.tex <==
\section{Continuous GWNN}

A major issue remains: what to do when there is no input signal? One may choose a constant input signal $z=1_n$, but remark that, in particular, when the degree function $d_W$ is constant, the output of \emph{any} equivariant GNN will tend to a constant vector.

In \cite{Vignac2020a} and \cite{Xu2019}, some authors propose a powerful architecture where each node is assigned a unique id (usually a one-hot vector), and equivariance is restored by a final node-wise pooling (akin to a "deep set" architecture). The authors in \cite{Vignac2020a} take inspiration from works \cite{Loukas2019} that prove that a unique id for each node leads to universality, while those of \cite{Xu2019} make a parallel with wavelets on graphs, that is, filtering of Dirac signals. They call the resulting network Graph Wavelets NN (GWNN).

Let us consider the equivariant case (the invariant is simpler). We define an equivariant GWNN as follows here. We consider any equivariant GCN $\Phi_A(\cdot): \RR^n \to \RR^{n \times d_{out}}$ as defined above (that is, with input dimension $d_0=1$). 
\begin{equation}
\Psi_A \eqdef \rho\left(\left(\frac{1}{n} \sum_i \Phi_A(e_i)\right) \tilde\theta \right) + 1_n \tilde b^\top \in \RR^{n \times d'_{out}}
\end{equation}
Where $e_i = [0,\cdot, 1, \cdot, 0]$ is the $i$th basis vector of $\RR^n$, $\tilde \theta \in \RR^{d_{out} \times d'_{out}}, \tilde b \in \RR^{d'_{out}}$ are the weights and bias of a MLP. In other words, $\Phi_A$ is applied to \emph{each} $e_i$, then a pooling is performed, and a final fully connected layer is done.

In particular, GWNN are invariant to the choice of ids $e_i$ in the first layer: we have $\frac{1}{n} \sum_i \Phi_A(e_i) = \frac{1}{n} \sum_i \Phi_A(e_{\sigma(i)})$ for any permutation. This makes the whole architecture globally equivariant: since $\Phi_{\sigma \cdot A}(\sigma \cdot z) = \sigma \cdot \Phi_A(z)$, it is easy to see that
\begin{align*}
\Psi_{\sigma \cdot A} = \sigma\cdot \Psi_A
\end{align*}

We know that $\Phi_A(z)$ "tends to" a (sampling of a) function $\Phi_{W,P}(f)$ when $z$ is a suitable sampling of $f$. Does the same holds for GWNN ? Well, intuitively, $e_i$ can be seen as a ``Dirac'' at $x_i$. So, one would expect them to tend to the function
\begin{equation}
\Psi_{W,P} = \rho\circ\left(\tilde \theta^\top\int  \Phi_{W,P}(\delta_x) dP(x)\right) + \tilde b
\end{equation}
with proba $1$, as long as "$\Phi_{W,P}(\delta_x)$" makes sense.

One can easily define the filtering of Diracs \emph{when there is no order-$0$ term}, by $\Ll_{W,P} \delta_x = \int \bar W(\cdot, x') d \delta_x(x') = \bar W(\cdot, x) \in \Bb(\Xx)$, and so on (recall that $\bar W = W(x,y)/\sqrt{d_W(x)d_W(y)}$ is just the normalized kernel used in the Laplacian). In fact, we will prove that the term of order $0$ in the first layer vanishes. For a filter $h(\lambda) = \sum_{k\geq 0} \beta_k \lambda^k$, we define $h^{\backslash 0} (\lambda) = \sum_{k \geq 0} \beta_{k+1} \lambda^k$, that is, all the coefficients are shifted.

Let $\Phi_A$ be an equivariant GCN. We define the following continuous architecture: for all $x$,
\begin{align*}
f^{(1)}_j (\cdot, x) &= \rho \circ \left( h_{0j}^{(0), \backslash 0}(\Ll_{W,P})[\bar W(\cdot, x)] + b^{(1)}\right) \\
f^{(\ell + 1)}_j (\cdot, x) &= \rho \circ \left( \sum_{i=1}^{d_\ell} h_{ij}^{(\ell)}(\Ll_{W,P})[f^{(\ell)}_i(\cdot, x)] + b^{(\ell)}_j \right) \\
\Phi_{W,P}(\cdot,x) &= \theta^\top f^{(M)}(\cdot, x) + b\\
\Psi_{W, P} &= \rho\circ\left(\tilde \theta^\top \int \Phi_{W,P}(\cdot, x) dP(x)\right) + \tilde b
\end{align*}
In other words, bivariate functions are manipulated, $\bar W$ is inputed, the filters at the first layers do not have an order-$0$ term, and a final integration is performed.

\paragraph{Convergence} We have the same result as before, with different constants.
\begin{theorem}[Convergence \textcolor{red}{to finish}]\label{thm:gwnn}
Take any $\rho>0$, assume $n$ is large enough such that $n \geq  ...$, and the sparsity level is such that $\alpha_n \geq O( n^{-1}\log n)$.
Then, with probability at least $1-\rho$,
\begin{align*}
\textup{MSE}_X\pa{\Psi_A, \Psi_{W,P}} &\leq O( n^{-\frac12}) + O( (n\alpha_n)^{-\frac12})
\end{align*}
\end{theorem}

\paragraph{Approximation power} Is this more powerful than before ? Yes: GWNN are more general than GCNs with constant input, since a constant input can be emulated by just taking the bias in the first layer and putting the weights to $0$. Moreover, the inclusion is strict: it is easy to build a model with constant degree function, where the output of any GCN is constant, but the output of GWNNs is not.

Let us outline a few examples.
%In the rest, we use $W$ or $ \bar W$ indiscriminately for simplicity. Consider the following $1$-layer GWNN:
%\begin{equation}
%\Psi_{W,P} = \int g_\theta(W(\cdot, x)) dP(x)
%\end{equation}
%where $g_\theta: \RR \to \RR$ is a MLP, so can approximate any function. If $W$ is a Gaussian kernel, $g_\theta(W)$ can be as spiky as wanted, and then one can perform "deconvolution" on $P$ and find a density $p(x)$ at each node, ie its relative importance. As another example,
Consider a SBM with two communities: $W_{11} = 1, W_{12} = 1/3, W_{22} = 2/3, \pi_1 = 1/3, \pi_2 = 2/3$. The degree is constant, so normal GCN cannot distinguish anything. However, the above architecture can be such as $g_\theta(W_{11}) = 3, g_\theta(W_{12}) = 0, g_\theta(W_{22}) =1$, such that $\Psi_{W,P}$ is $1$ at nodes in community $1$ and $2/3$ at nodes in community $2$, and so can easily classify them.

\begin{proof}[Proof of Theorem \ref{thm:gwnn}]

We denote by $Z^{(\ell)}(e_q)$ the intermediate layer of $\Phi_A(e_q)$. Also denote the discrete GCN without order-$0$ term:
\begin{align*}
z^{(0)}(x_q) &= [\bar W(x_i, x_q)]_i = L e_q \\
z^{(1)}_j (x_q) &= \rho \left( h_{1j}^{(0), \backslash 0}(L)z^{(0)}(x_q) + b^{(1)}1_n\right) \\
z^{(\ell + 1)}_j (x_q) &= \rho \left( \sum_{i=1}^{d_\ell} h_{ij}^{(\ell)}(L) z^{(\ell)}_i(x_q) + b^{(\ell)}_j 1_n\right)
\end{align*}
and aggregated $Z^{(\ell)}(x_q)$.

We decompose the error:
\begin{align*}
MSE_X(\Psi_A , \Psi_{W,P}) &= \sqrt{\frac{1}{n} \sum_i \abs{\rho\left(\frac{1}{n} \sum_q (Z^{(M)}(e_q) \theta)_i + b\right)\tilde\theta - \rho\left(\int \theta^\top f^{(M)}(x_i, x) dP(x) + b\right) \tilde\theta}^2} \\
&\leq \norm{\theta} \norm{\tilde\theta}\norm{\frac{1}{n} \sum_q \frac{Z^{(M)}(e_q)}{\sqrt{n}} - S_X\int f^{(M)}(\cdot, x) dP(x)}_F \\
&\leq \norm{\theta}\norm{\tilde\theta}\Big( \norm{\frac{1}{n} \sum_q \frac{Z^{(M)}(e_q)}{\sqrt{n}} - \frac{Z^{(M)}(x_q)}{\sqrt{n}}}_F \\
&\quad + \sup_x \norm{\frac{Z^{(M)}(x)}{\sqrt{n}} - S_X f^{(M)}(\cdot, x)}_F \\
&\quad + \sup_y \norm{\frac{1}{n} \sum_q f^{(M)}(y, x_q) - \int f^{(M)}(y, x) dP(x)} \Big)
\end{align*}
So the error has three terms. The first comes from the removal of the order-$0$ term in the first layer, should be trivial. The third is a uniform concentration inequality that can be handled with chaining under proper regularity assumptions. The second is similar to the previous core of the proof, but will probably ask for "bivariate" chaining concentration inequalities, which should be fine.

\paragraph{First error term}
Using tools from previous proof, for each $q$, for $\ell\geq 1$ we bound
\begin{align*}
\norm{Z^{(\ell+1)}(e_q) - Z^{(\ell+1)}(x_q)}_F &= \left(\sum_j \norm{ \rho \left( \sum_i h_{ij}^{(\ell)}(L) z^{(\ell)}_i(e_q) + b_j^{(\ell)}1_n \right) - \rho \left( \sum_i h_{ij}^{(\ell)}(L) z^{(\ell)}_i(x_q)  + b_j^{(\ell)}1_n \right) }^2 \right)^\frac12 \\
&\leq \left(\sum_j \norm{ \sum_i h_{ij}^{(\ell)}(L) (z^{(\ell)}_i(e_q) - z^{(\ell)}_i(x_q))}^2 \right)^\frac12  \leq H_2^{(\ell)} \norm{Z^{(\ell)}(e_q) - Z^{(\ell)}(x_q)}_F
\end{align*}
and for $\ell=0$: since $h_{1j}^{(0)}(L) e_q = h_{1j}^{(0),\backslash 0}(L) L e_q + \beta_{1j0} e_q$,
\begin{align*}
\norm{Z^{(1)}(e_q) - Z^{(1)}(x_q)}_F &= \left(\sum_j \norm{ \rho \left( h_{1j}^{(0)}(L) e_q + b_j^{(0)}1_n \right) - \rho \left( h_{1j}^{(0),\backslash 0}(L) L e_q  + b_0^{(\ell)}1_n \right) }^2 \right)^\frac12 \leq \norm{(\beta_{1 j 0})_j} \eqdef C_0
\end{align*}
So, the first error is bounded by $\frac{C_0\prod H_2^{(\ell)}}{\sqrt{n}}$.

\paragraph{Third error term}
The third error can be bounded using chaining. Applying Lemma \ref{lem:chaining-pointwise}, if $f^{(M)}$ is $C_f$-bounded and $(n_f, C'_f)$-Lipschitz, with probability $1-\rho$ the third error term is bounded by (\textcolor{red}{Todo: compute constants, clean multivariate chaining})
\begin{equation}
\frac{C'_f \sqrt{d_x} + (C_f + C'_f)\sqrt{\log\frac{n_f}{\rho}}}{\sqrt{n}}
\end{equation}

\paragraph{Second error term} This can be done with chaining on the product space

\end{proof}
